Complexity and Inapproximability Results for Parallel Task Scheduling and Strip Packing

We study the Parallel Task Scheduling problem $Pm|size_j|C_{\max}$ with a constant number of machines. This problem is known to be strongly NP-complete for each $m \geq 5$, while it is solvable in pseudo-polynomial time for each $m \leq 3$. We give a positive answer to the long-standing open question whether this problem is strongly $NP$-complete for $m=4$. As a second result, we improve the lower bound of $\frac{12}{11}$ for approximating pseudo-polynomial Strip Packing to $\frac{5}{4}$. Since the best known approximation algorithm for this problem has a ratio of $\frac{4}{3} + \varepsilon$, this result narrows the gap between approximation ratio and inapproximability result by a significant step. Both results are proven by a reduction from the strongly $NP$-complete problem 3-Partition.

==> reduction.tex <==
In the following we will proof Theorem \ref{thm:hardness} by a reduction from the 3-Partition problem. We will show that if we can decide if the optimal packing height of a strip packing instance $\mathcal{I} = (I,W)$ is $4$ in time polynomial in $W$ and $|I|$, we can solve the 3-Partition problem as well.

In the 3-Partition problem we have given a list $\mathcal{A} = (a_1,\dots,a_{3z})$ of $3z$ integers, such that $\sum_{i = 1}^{3z}a_i = zD$ and $D/4 < a_i < D/2$ for each $1\leq i \leq 3z$. The problem is to decide if there exists a partition of the set $I = \{1,\dots,3z\}$ into sets $I_1, \dots I_z$, such that $\sum_{i \in I_j} a_i = D$ for each $1 \leq j \leq z$.

This problem is strongly NP-complete \cite{GareyJ79}. Therefore, we can not solve it in polynomial time of the size of the input, even if the numbers $a_1, \dots a_{3z}$ are given in unary. 

\paragraph{Construction}
First we will describe how we generate a strip packing instance $\mathcal{I} =(I,W)$ from a given 3-partition instance $\mathcal{A}$ in polynomial time. Let $\mathcal{A}  = (a_1,\dots,a_{3z})$ be a 3-partition instance, with $\sum_{i = 1}^{3z}a_i = zD$. If $D \leq \scalePart$ we scale each number with $\scalePart$ such that we get a new instance $\mathcal{A} ' := (\scalePart \cdot a_1,\dots,\scalePart \cdot a_{3z})$. For this instance it holds that $D' = \scalePart D> \scalePart$ and $SIZE(\mathcal{A} ') \in \mathrm{poly}(SIZE(\mathcal{A} ))$. Therefore, let us w.l.o.g assume that $D > \scalePart$.

In the following we describe the items we construct in this reduction, see Figure \ref{fig:overviewItems} for an overview. We generate two sets $A$ and $B$ of items with height $3$. $A$ contains $z+1$ items with width $D^2$ and $B$ contains $z+1$ items with width $D^3$. 
Furthermore we generate three sets $a$, $b$ and $c$ with items with height 2, such that $a$ contains $z$ items with width $D^4 + D^6 +3zD^7$, $b$ contains $z$ items with width $D^5 + D^6 + 3zD^7$ while $c$ contains one item for each $0 \leq i \leq z$, having width $(z+i)D^7 + D^8$ resulting in $z+1$ items total. 
Last we define five sets $\alpha$, $\beta$, $\gamma$, $\delta$, and $\lambda$ of items width height 1, such that 
$\alpha$ contains $z$ items with width $D^3 + D^5 + 4zD^7 +D^8$, 
$\beta$ contains $z$ items with width $D^2 + D^4 + (4z-1)D^7 +D^8$, 
$\gamma$ contains for each $1 \leq i \leq z$ one item with width $D^5 + (3z -i)D^7 -D$ resulting in $|\gamma| = z$, 
$\delta$ contains for each $1 \leq i \leq z$ one items with width $ D^4 + (3z -i)D^7$ resulting in $|\delta| = z$, 
and $\lambda$ contains two items $\lambda_1$ and $\lambda_2$ with $w_{\lambda_1} = D^3 + zD^7 + D^8$ and $w_{\lambda_2} = B+ c_0 = D^2 + 2zD^7 + D^8$.
We call these items \textit{structure items}.
Additionally we generate for each number $a_i$ out of $A = (a_1,\dots,a_{3z})$ a \textit{partition item}, which has height 1 and width $a_i$. We name the set of partition items $P$.


\begin{figure}[ht]

\begin{align*}
w_i = 
\begin{cases}
D^2 & i \in A\\
D^3 & i \in B\\
D^4 + D^6 +3zD^7 & i \in a,\\
D^5 + D^6 +3zD^7 & i \in b,\\
(z+j)D^7 + D^8 & i = c_j\in c, j\in \{0,\dots,z\}\\
D^3 + D^5 + 4zD^7 +D^8 &  i \in \alpha\\
D^2 + D^4 + (4z-1)D^7 +D^8 &  i \in \beta\\
D^5 + (3z -j)D^7 -D & i = \gamma_j \in \gamma, j\in \{1,\dots,z\}\\
D^4 + (3z -j)D^7 & i = \delta_j \in \delta, j\in \{1,\dots,z\}\\
D^3 + zD^7 + D^8 &  i = \lambda_1\\
D^2 + 2zD^7 + D^8 &  i = \lambda_2\\
\end{cases}
\end{align*}
\caption{Overview of the structure items}
\label{fig:overviewItems}
\end{figure}

We define the width of the strip as $W := (z+1)(D^2 + D^3 +D^8) + z(D^4 + D^5 +D^6) + z(7z + 1)D^7$. Note that the area of the items adds up to $4 W$. Therefore, an optimal packing has height at least 4 and each packing of height 4 contains no free area (i.e it is optimal).

\newpage
\paragraph{Partition to Packing} 
Let $A$ be a yes-instance with partition $I_1, \dots, I_z $.
One can easily verify that the \textit{structure items} can be placed as shown in Figure \ref{fig:packingStructure}. Left of each item $\gamma_j$, for each $1 \leq j \leq z$, we have a gap with width $D$. We place the \textit{partition items} with indices out of $I_j$ left of $\gamma_j$. Their widths add up to $D$, therefore they fit into the gap. The resulting packing has a height of $4$. Since there is no free area left in the packing, it is optimal.
\begin{figure}[ht]
\centering
\begin{tikzpicture}
\pgfmathsetmacro{\h}{0.5}
\pgfmathsetmacro{\w}{0.5}

\draw (-3*\w,0*\h) rectangle node[midway]{$\lambda_1$}(0*\w,1*\h);

\foreach \y in {1,2} { 
\pgfmathsetmacro{\x}{\y - 1}
\begin{scope}[xshift = 9*\h*\x cm]
\draw (-2*\w,3*\h) rectangle node[midway]{$\beta$}(3*\w,4*\h);
\draw (0,0) rectangle node[midway]{$A$}(1*\w,3*\h);
\draw (1*\w,0) rectangle node[midway]{$a$}(4*\w,2*\h);
\draw (3*\w,2*\h) rectangle node[midway]{$b$}(6*\w,4*\h);
\draw (-3*\w,1*\h) rectangle node[midway]{$B$}(-2*\w,4*\h);
\draw (1*\w,2*\h) rectangle node[midway]{$\delta_{\y}$}(3*\w,3*\h);
\draw (4*\w,1*\h) rectangle node[midway]{$\gamma_{\y}$}(5.5*\w,2*\h);
\draw[pattern = north west lines] (5.5*\w,1*\h) rectangle (6*\w,2*\h);
\draw (4*\w,0*\h) rectangle node[midway]{$\alpha$}(9*\w,1*\h);
\end{scope}
}

\foreach \y in {0,1} { 
\begin{scope}[xshift = 9*\h*\y cm]
\draw (-2*\w,1*\h) rectangle node[midway]{$c_{\y}$}(0*\w,3*\h);
\end{scope}
}

\node at (17*\w, 2.5*\h) {$\dots$};

\begin{scope}[xshift = 2*\w cm, yshift = -5*\h cm]
\foreach \y in {2,1} { 
\pgfmathsetmacro{\x}{-\y +2}
\begin{scope}[xshift = 9*\w*\x cm]
\draw (-2*\w,3*\h) rectangle node[midway]{$\beta$}(3*\w,4*\h);
\draw (0,0) rectangle node[midway]{$A$}(1*\w,3*\h);
\draw (1*\w,0) rectangle node[midway]{$a$}(4*\w,2*\h);
\draw (3*\w,2*\h) rectangle node[midway]{$b$}(6*\w,4*\h);
\draw (-3*\w,1*\h) rectangle node[midway]{$B$}(-2*\w,4*\h);
\draw[pattern = north west lines] (5.5*\w,1*\h) rectangle (6*\w,2*\h);
\draw (4*\w,0*\h) rectangle node[midway]{$\alpha$}(9*\w,1*\h);
\draw (-2*\w,1*\h) rectangle node[midway]{$c_{z-\y}$}(0*\w,3*\h);
\end{scope}
}


\begin{scope}[xshift = 9*\w*2 cm]
\draw (-3*\w,1*\h) rectangle node[midway]{$B$}(-2*\w,4*\h);
\draw (-8*\w,2*\h) rectangle node[midway]{$\delta_{z}$}(-6*\w,3*\h);
\draw (-5*\w,1*\h) rectangle node[midway]{$\gamma_{z}$}(-3.5*\w,2*\h);
\draw (-2*\w,1*\h) rectangle node[midway]{$c_{z}$}(0*\w,3*\h);
\draw (0,0) rectangle node[midway]{$A$}(1*\w,3*\h);
\end{scope}


\draw (1*\w,2*\h) rectangle node[midway]{$\delta_{z-1}$}(3*\w,3*\h);
\draw (4*\w,1*\h) rectangle node[midway]{$\gamma_{z-1}$}(5.5*\w,2*\h);
\end{scope}

\draw (18*\w,-2*\h) rectangle node[midway]{$\lambda_2$}(21*\w,-1*\h);
\node at (-2*\w, - 2.5*\h) {$\dots$};
%\draw (25*\w,3*\h) rectangle node[midway]{$\lambda_2$}(28*\w,4*\h);
%\draw (27*\w,0) rectangle node[midway]{$A$}(28*\w,3*\h);

\node at (-4.5*\w,0.5 *\h) {slot 1};
\node at (-4.5*\w,1.5 *\h) {slot 2};
\node at (-4.5*\w,2.5 *\h) {slot 3};
\node at (-4.5*\w,3.5 *\h) {slot 4};
\end{tikzpicture}
\caption{An optimal packing, for a yes-instance}
\label{fig:packingStructure}
\end{figure}


\paragraph{Packing to Partition}
We will show that each packing with height $4$ looks similar to the packing in Figure \ref{fig:packingStructure}.\footnote{TODO: beschreiben, dass es keinen übertrag geben kann}
First, we will show that the four slots contain the same items as in Figure \ref{fig:packingStructure}.

Let $I' \subseteq I$ be a set of structure items. Notice that their total width $w(I)$ is always of  the form $\sum_{i = 2}^8x_i D^i$, for some values $x_i \in \mathbb{N}_{\leq \scalePart}$. Since $\scalePart < D$ it can not happen, that by adding enough items we lift up one $x_i D^i$ to the next higher exponent.

\begin{lma}
Let a packing of $I$ with height $4$ be given. Then slot 1 contains all items in $A \cup a \cup \alpha \cup \{\lambda_1\}$, slot 2 contains all items in $A \cup B \cup a \cup c \cup \gamma \cup P$, slot 3 contains all items in $A \cup B \cup b \cup c \cup \delta$, and slot 4 contains all items in $B \cup b \cup \beta \cup \{\lambda_2\}$, or the content of the slots 1 and 4 is swapped as well as the content of the slots 2 and 3.
\end{lma}
\begin{proof}
Let us first look at the items in the sets $A$ and $B$. These items have height $3$. Therefore the only two possible $y$-positions for these items are $0$ and $1$. At each larger number the packing would have a height larger than $4$. In either case the items are contained in the slots 2 and 3. Furthermore each item in $A \cup B$ is either contained in slot 1 or slot 4.

Next we will show that the items in the set $\alpha \cup \beta \cup \{\lambda_1, \lambda_2\}$ have to be contained in the slots 1 and 4.
The slots 2 and 3 both contain all the items in $A \cup B$. 
The widths of these items add up to a total of $(z+1)D^2 + (z+1)D^3$. Therefore no other item with a width containing $D^2$ or $D^3$ can be contained in slot 2 an 3. Each item in the set $\alpha \cup \beta \cup \{\lambda_1, \lambda_2\}$ has a width, which contains $D^2$ or $D^3$.  
Consequently, the slots 1 and 4 contain all the items from $\alpha \cup \beta \cup \{\lambda_1, \lambda_2\}$ as well as one part from each item in $A \cup B$. 

In the next step we will see that one part of each item in $a \cup b$ is contained by slot 1 and 4.
The total area of the items we have so far proven to be contained by slots 1 and 4 adds up to $2(z+1)D^2 + 2(z+1)D^3 + zD^4 + zD^5 + 2z(4 z +1) D^7 + 2(z+1)D^8$. 
To fill slots 1 and 4, items with a total width of $zD^4 + zD^5 + 2zD^6 + 6zD^7$ are missing. The only items, whose width contains $D^6$ are the items in the sets $a$ and $b$. 
In total these sets contain $2z$ items. 
Since each item in these sets has a height of 2, they can either be contained in slot 1 or slot 4 but not in both at once. 
We need $2z$ of $D^6$ and each of the items in $a$ and $b$ adds one $D^6$. Therefore, all the items in $a$ and $b$ have to be contained either in slot 1 or in slot 4. 
In total the slots 1 and 4 contain all the items from $\alpha \cup \beta \cup \{\lambda_1, \lambda_2\}$ as well as one part from each item in $A$, $B$, $a$, and $b$. The areas of these item (parts) add up to $2W$.

Now, we will show that the only possibility to partition the set of items parts contained in slots 1 and 4 such that their width adds up to $W$ is the partition $\{A \cup a \cup \alpha \cup \{\lambda_1\}, B \cup b \cup \beta \cup \{\lambda_2\}\}$.
Let us look at the coefficient of $D^7$. The items in the sets $a$ and $b$ add the same amount of $D^7$ and  $D^6$ to the area. Therefore, $z$ item parts out of $a \cup b$ have to be contained in slot 1 and the same number in slot 4. These items add a total of $3z^2D^7$ to each slot. 
So we have left an amount of $z(4z+1)D^7$ per slot. The only other items, which have a width containing $D^7$ are the items in $\alpha \cup \beta \cup \{\lambda_1, \lambda_2\}$. Since each of these items has a width which contains one $D^8$ one slot can contain at most $z+1$ of these items, the other $z+1$ have to be contained in the other slot. 
Let w.l.o.g. slot 1 contain $\lambda_1$. So this slot is missing $(z(4z+1)-z)D^7 = 4z^2D^7$. So slot 1 has to contain $z$ further items from $\alpha \cup \beta \cup \{\lambda_2\}$, with an amount of $D^7$ adding up to $4z^2D^7$. The items in $\alpha$ have the largest amount of $D^7$. 
The amount of $D^7$ in all the $z$ items in $\alpha$ adds up too $4z^2$. So slot 2 has to contain all the items in $\alpha$, since otherwise the amount of $D^7$ would be too small. 
This means the items in $\beta \cup \{\lambda_2\}$ are contained in slot 4. 
Besides the items in $\alpha \cup \{\lambda_1\}$ slot 1 has to contain items with a total width of $(z+1)D^2 + zD^4 + zD^6 + 3z^2D^7$. 
The only set of items contained in slot 1 and 4 and not already contained in slot 4, which sums up to this width is the set $A \cup a$. 
So slot 1 contains the set $A \cup a \cup \alpha \cup \{\lambda_1\}$, while slot 4 contains the set $B \cup b \cup \beta \cup \{\lambda_2\}$. 

As a consequence, slot 2 contains the set $A \cup B \cup a \cup c$, while slot 3 contains all items in $A \cup B \cup b \cup c$. Slot 3 is missing $z$ items, with a width containing $D^4$. The only items left which contain $D^4$ in their width are the items in the set $\delta$. Therefore slot 3 has to contain all the items in $\delta$. As a consequence all the items in the set $\gamma \cup P$ have to be contained in slot 2, since there is no free area left on slot 3.
\end{proof}

Let us from now on assume, that the slots contain the same items as in Figure \ref{fig:packingStructure}. 
In the next step we will show, that the items have to appear in the same order from left to right as the items in Figure \ref{fig:packingStructure}. Let us first notice, that an $x$ coordinate of an item $i$ has to be the sum of the width of the items placed left of $i$ in the same slot, since there is no free area in any slot. So the $x$ coordinate of any item has to be of the form 
\[x_1 + x_2D^2 + x_3D^3 + x_4D^4 + x_5D^5 + x_6D^6 + x_7D^7 + x_8D^8\]
where $|x_1| < D^2$ and $0 \leq x_j < D$ for each $2 \leq j \leq 8$. This allows us to make conclusions about the correlation of the number of occurrence of items appearing left of a placed item on different slots. For example, we know that the only items which increase $x_5$ are the items in the sets $\alpha$, $\gamma$ and $b$. Furthermore items in $\alpha$ are just contained in slot 1, items in $\gamma$ are just contained in slot 2 and items in $b$ are just contained in slots 3 and 4. Therefore, we know that, if an item $i \in A$ is placed at position $(x_i,y_i)$, the number of items out of $\alpha$ positioned left of $x_i$ equals the number of items out of $\gamma$ positioned left of $x_i$, which equals the number of items out of $b$ positioned left of $x_i$, since each item out of $A$ is contained in slots 1, 2 and 3.

In Table \ref{table:occ1} and \ref{table:occ2} we display our knowledge about which items increase the coefficient $x_j$, if it occurs left of the position $x_i = x_1 + x_2D^2 + x_3D^3 + x_4D^4 + x_5D^5 + x_6D^6 + x_7D^7 + x_8D^8$.%\footnote{TODO: Tabelle erklären}

\begin{table}[ht]
\centering
\begin{tabular}{c|ccc}
A & slot 1 & slot 2 & slot 3\\
\hline
$x_3$&$\#\alpha + \#\{\lambda_1\}$&$\#B$&$\#B$\\
$x_4$&$\# a$&$\# a$&$\#\delta$\\
$x_5$&$\#\alpha$&$\#\gamma$&$\#b$\\
$x_6$&$\# a$&$\# a$&$\# b$\\
$x_8$&$\# \alpha +\# \{\lambda_1\}$&$\#c$&$\#c$\\
\end{tabular}
\hspace{2em}
\begin{tabular}{c|ccc}
B & slot 2 & slot 3 & slot 4\\
\hline
$x_2$&$\#A$&$\#A$&$\#\beta + \#\{\lambda_2\}$\\
$x_4$&$\# a$&$\#\delta$&$\#\beta$\\
$x_5$&$\#\gamma$&$\# b$&$\# b$\\
$x_6$&$\# a$&$\#b$&$\#b$\\
$x_8$&$\# c$&$\# c$&$\#\beta + \#\{\lambda_2\}$\\
\end{tabular}
\caption{correlation of item occurrences, when an item $i \in A$ or $i \in B$ is placed}
\label{table:occ1}
\end{table}

\begin{table}[ht]
\centering
\begin{tabular}{c|cc}
a & slot 1 & slot 2 \\
\hline
$x_3$&$\#\alpha + \#\{\lambda_1\}$&$\#B$\\
$x_5$&$\#\alpha$&$\#\gamma$\\
$x_8$&$\# \alpha +\# \{\lambda_1\}$&$\#c$\\
\end{tabular}
\hspace{1em}
\begin{tabular}{c|cc}
b & slot 3 & slot 4\\
\hline
$x_2$&$\#A$&$\#\beta + \#\{\lambda_2\}$\\
$x_4$&$\# \delta$&$\#\beta$\\
$x_8$&$\# c$&$\#\beta + \#\{\lambda_2\}$\\
\end{tabular}
\hspace{1em}
\begin{tabular}{c|cc}
a & slot 2 & slot 3\\
\hline
$x_4$&$\# a$&$\# \delta$\\
$x_5$&$\#\gamma$&$\#b$\\
$x_6$&$\# a$&$\# b$\\
\end{tabular}
\caption{correlation of item occurrences, when an item $i \in a$, $i \in b$ or $i \in c$ is placed}
\label{table:occ2}
\end{table}

At the position where an item $i \in A$ is placed, we know that 
\begin{equation}
\label{align:xPositionA}
\#B - \#\{\lambda_1\}\overset{x_3}{=} \# \alpha \overset{x_5}{=} \# \gamma \overset{x_5}{=}\#b\overset{x_6}{=} \# a \overset{x_4}{=} \# \delta = \#c - \#\{\lambda_1\}.
\end{equation}
Furthermore we know that at the position of an item $i \in B$ we have
\begin{equation}
\label{align:xPositionB}
\# A - \# \{\lambda_2\} \overset{x_2}{=} \#\beta \overset{x_4}{=} \# \delta \overset{x_4}{=} \# a \overset{x_6}{=} \# b \overset{x_5}{=} \#\gamma = \#c -\#\{\lambda_2\}.
\end{equation}
%\footnote{Beachte die Symmetrie: $\alpha \leftrightarrow \beta$, $a \leftrightarrow b$, $\delta \leftrightarrow \gamma$, $A \leftrightarrow B$, $\lambda_1 \leftrightarrow \lambda_2$ (spiegeln sowohl senkrecht als auch wagerecht)}
If we look at the items out of $a$, $b$ or $c$ we know slightly less, since these items have just height $2$. For an item $i \in a$ we know, that 
\begin{equation}
\label{align:xPositiona}
\#B - \#\{\lambda_1\}\overset{x_3}{=} \# \alpha \overset{x_5}{=} \# \gamma = \#c - \#\{\lambda_1\},
\end{equation}
while for an item $i \in b$ we have
\begin{equation}
\label{align:xPositionb}
\# A - \# \{\lambda_2\} \overset{x_2}{=} \#\beta \overset{x_4}{=} \# \delta = \#c -\#\{\lambda_2\}.
\end{equation}
%\footnote{Hier die gleiche Symmetrie}
For each item $i \in c$ we have
\begin{equation}
\label{align:xPositionc}
\#\delta \overset{x_4}{=}\# a \overset{x_6}{=}\# b \overset{x_5}{=}\# \gamma.
\end{equation}

These properties allow the following conclusions:

\begin{lma}
The left most item and the rightmost item in slots $2$ and $3$ are elements of $A \cup B$.
\end{lma}
\begin{proof}
%Let $i_0 \in I$ be the first item in slot $3$. Let $A_1 \in A$ be left most item in $A$ and $B_1 \in B$ be the leftmost item in $B$ contained in slot $3$. Let us for contradiction assume that $i_0 \not \in A \cup B$. Since slot $3$ contains the items $A \cup B \cup c \cup a \cup \delta$ it follows that $i_0 \in c$, $i_0 \in a$ or $i_0 \in \delta$. In the following we will disprove all of these possibilities.
%
%Let us assume that $i_0 \in c$. 
%It holds that 
%$\#_{A_1} B =_{(\ref{align:xPositionA})} \#_{A_1} c \geq 1$.
%As a consequence $B_1$ has to be positioned left of $A_1$. Furthermore, it holds that 
%$\#_{B_1} A =_{(\ref{align:xPositionB}) } \#_{B_1} c \geq 1$. 
%As a consequence $A_1$ has to be positioned left of $B_1$, a contradiction. Thus $i_0 \not \in c$.
%
%Let us assume that $i_0 \in a$.
%It holds that $\#_{A_1}B - \#_{A_1}\{\lambda_1\}=_{(\ref{align:xPositionA})}\#_{A_1} a \geq 1$. Since $\#_{A_1}\{\lambda_1\} \in \{0,1\}$, it follows that $\#_{A_1}B \geq 1$, which means $B_1$ has to be placed left of $A_1$. Analogously equality (\ref{align:xPositionB}) demands that $\#_{B_1} A - \#_{B_1}\{\lambda_2\} = \#_{B_1} a$. Since $\#_{B_1}\{\lambda_2\} \in \{0,1\}$, it follows that $\#_{B_1} A \geq \#_{B_1} a \geq 1$, which means that $A_1$ has to be positioned left of $B_1$ contradicting the assumption. Hence $i_0 \not \in a$.
%
%Analogously we can disprove the assumption that $i_0 \in \delta$. Since slot $3$ contains the items $A \cup B \cup a \cup c \cup \delta$ and $i_0 \not \in  a \cup c \cup \delta$, it follows that $i_0 \in A \cup B$.
%%The only possibilities remaining are the items out of $A \cup B$. 
%Since each packing can be mirrored at the y-axis and stays feasible, the rightmost item in slot $3$ is out of $A \cup B$ as well.

Let $i := \arg\min_{i \in A \cup B} x_i$ be the item with the left most position  in $A \cup B$, (i.e. $\#_{i} A = \#_{i} B = 0$). We have to consider each case $i \in A$ and $i \in B$ and to show that $\rho(i)$ has the x-coordinate $x_i = 0$. 

First case: $i \in A$. In this case it holds that $\#_{i} a + \#_{i}\{\lambda_1\} =_{(\ref{align:xPositionA})} \#_{i}\alpha + \#_{i}\{\lambda_1\} =_{(\ref{align:xPositionA})} \#_{i}B = 0$ and therefore $\#_{i}\alpha = 0$ as well as $\#_{i}\{\lambda_1\} = 0$ and $\#_{i} a = 0$. The items $a \cup \alpha \cup \{\lambda_1\} \cup A$ are the only items, which are contained in slot $1$. Since $\#_{i}a =\#_{i} \alpha = \#_{i} \{\lambda_1\} = \#_{i} A =0$ it has to be that $s_i = 0$ and therefore $i$ is the leftmost item in the slots $2$ and $3$.

Second case: $i \in B$. In this case it holds that $ \#_{i} b + \#_{i}\{\lambda_2\} =_{(\ref{align:xPositionB})} \#_{i}\beta + \#_{i}\{\lambda_2\} =_{(\ref{align:xPositionB})} \#_{i}A = 0$ and therefore $\#_{i}\beta = 0$, $\#_{i}\{\lambda_2\} = 0$ and $\#_{i} b = 0$. The items $b \cup \beta \cup \{\lambda_2\} \cup B$ are the only items, which are contained in slot $4$. Since $\#_{i}b =\#_{i} \beta = \#_{i} \{\lambda_2\} = \#_{i} B = 0$ it has to be that $s_i = 0$ and therefore $i$ is the leftmost item on slots $2$ and $3$.

So we have shown that the leftmost item on slots $2$ and $3$ hast to be a job from the set $A \cup B$. Since the schedule stays valid, if we mirror the schedule such that the last job is the first job and the first job is the last job, the last job has to be in the set $A \cup B$ as well.
\end{proof}

We can w.l.o.g. assume that the first item on slot 3 is an item out of $B$, since we will prove that in this case the last one will be an item out of $A$.

\begin{lma}
If the first item on slot 2 is an item out of $B$ it holds for each item $i \in A$ that 
\begin{equation}
\#_{i} B - \#_{i}\{\lambda_1\} = \#_i A
\label{equ:relationAB}
\end{equation}
and $\#_{i}\{\lambda_1\} = 1$.
\end{lma}
\begin{proof}
We will show this claim inductively.
Let $(A_0, \dots, A_{z})$ be the set $A$ and $(B_0, \dots, B_{z})$ be the set $B$ each ordered by increasing size of the $x$-coordinate.
%Let $A_1 \in A$ be the leftmost job in slot 2. 

Assume $\#_{A_0} B - \#_{A_0}\{\lambda_1\} > \#_{A_0}A = 0$. Equality (\ref{align:xPositionA}) assures that 
$1 \leq \#_{A_0} B - \#_{A_0}\{\lambda_1\} = \#_{A_0} a = \#_{A_0} b = \#_{A_0} c - \#_{A_1}\{\lambda_1\}.$
As a consequence, there are positioned at least one item $a' \in a$, one item $b' \in b$ and one item $c'\in c$ left of $A_1$. Let $a'$, $b'$ and $c'$ be the leftmost items from their sets. 
Equality (\ref{align:xPositionb}) ensures that 
$ 0 = \#_{b'} A  =_{(\ref{align:xPositionb})} \#_{b'} c$.
Therefore $b'$ is positioned left of $c'$.  
Equality (\ref{align:xPositiona}) ensures that 
$\#_{a'}c =_{(\ref{align:xPositiona})} \#_{a_1}B \geq 1$.
Therefore $c'$ has to be placed left of $a'$. 
Summarizing we have 
$0 = \#_{c'}a =_{(\ref{align:xPositionc})}\#_{c'} b \geq 1$,
a contradiction. So we have shown that $\#_{A_0} B - \#_{A_0}\{\lambda_1\} \leq \#_{A_0}A.$
It can not be that $\#_{A_1} B - \#_{A_1}\{\lambda_1\} < 0$, since
$\#_{A_1} B \geq 1$ and $\#_{A_1}\{\lambda_1\} \in \{0,1\}$.
It follows that  $\#_{A_1} B - \#_{A_1}\{\lambda_1\} = 0 = \#_{A_0}A$ and therefore $\#_{A_1}\{\lambda_1\}=1$, $\#_{A_1}\alpha=0$ and $\#_{A_1} a = 0$.


Choose $i \in \{0,\dots z\}$ such that $\#_{A_{i'}} B - \#_{A_{i'}}\{\lambda_1\} = \#_{A_{i'}} A$ for each $i' \leq i$. Equality (\ref{align:xPositionA}) and $\#_{A_1}\{\lambda_1\}=1$ induce that $\#_{A_{i'}} A =\#_{A_{i'}} B -1 = \#_{A_{i'}} a = \#_{A_{i'}} b = \#_{A_{i'}} c -1$. Furthermore, we have $\#_{B_{i}} B = i = \#_{A_{i}} A = \#_{A_{i}} B -1$. Therefore $B_i$ has to be scheduled before $A_i$. Additionally, we have $\#_{B_{i}} B-1=\#_{B_{i-1}} B= i-1=\#_{A_{i-1}} A = \#_{A_{i-1}} B -1$, so $B_i$ has to be scheduled after $A_{i-1}$. Therefore we have 
\begin{equation}
\#_{B_{i}} B = \#_{B_{i}} A.
\label{align:AB}
\end{equation}

Assume that $\#_{A_{i+1}} B - \#_{A_{i+1}}\{\lambda_1\} > \#_{A_{i+1}} A$. 
It follows that $(\#_{A_{i+1}} B - \#_{A_{i+1}}\{\lambda_1\}) - (\#_{A_i} B - \#_{A_i}\{\lambda_1\})\geq 2$
demanding that between $A_i$ and $A_{i+1}$ there are positioned at least 2 items from the sets $B$, $a$, $b$ and $c$. We will refer to these items as $X', X'' \in X$, for $X \in \{B,a,b,c\}$, where $X'$ is positioned left of $X''$. We will now see how these items have to be arranged in the packing.
Both elements $b'$ and $b''$ are positioned left of $c'$, since 
\[\#_{A_i} c =_{(\ref{align:xPositionA})}\#_{A_i} A +1 = \#_{b''}A =_{(\ref{align:xPositionb})} \#_{b''} c.\] 
As a consequence, $a'$ and $a''$ have to be positioned left of $c'$ as well, since 
\[\#_{c'} a =_{(\ref{align:xPositionc})} \#_{c'} b \geq \#_{A_i} b +2 =_{(\ref{align:xPositionA})}  \#_{A_i} a +2.\]
%At every position where an element out of $c$ is placed, it holds that $\# a = \#b$ and we have $\#_{A_i} b = \#_{A_i} a$. 
%Therefore both elements $a'$ and $a''$ have to be placed left of $c'$ as well. 
As result, we have 
\[\#_{a''} B =_{(\ref{align:xPositiona})} \#_{a''} c = \#_{A_{i}} c =_{(\ref{align:xPositionA})}  \#_{A_{i}} B,\]
so both items $a'$ and $a''$ have to be placed left of  $B'$.
Furthermore $B''$ has to be placed left of $c'$, since 
\[\#_{B''} c  =_{(\ref{align:xPositionB})} \#_{B''}A = \#_{A_i}A+1 = \#_{A_i}B =_{(\ref{align:xPositionA})} \#_{A_i} c.\]
To this point we have deduced that the items appear in this order from left to right: $A_i, a', a'',B', B'', c',c'',A_{i+1}$. 
This placement is not feasible, since for this packing it holds that 
\[\#_{A_i} a +2 =\#_{B'}a \leq_{(\ref{align:xPositionB})} \#_{B'} A = \#_{A_i}A +1 =_{(\ref{align:xPositionA})} \#_{A_i} a +1,\] 
a contradiction. Hence we have $\#_{A_{i+1}} B - \#_{A_{i+1}}\{\lambda_1\} \leq \#_{A_{i+1}} A$.

%In total we have shown that for each item $i \in A$ we have $\#_{i} B - \#_{i}\{\lambda_1\} \leq \#_i A$. Thanks to the symmetry in the equations (\ref{align:xPositionA}) and (\ref{align:xPositionB}) as well as (\ref{align:xPositiona}) and (\ref{align:xPositionb}) we can analogously show that for each item $i \in A$ we have $\#_{i} B - \#_{i}\{\lambda_1\} \geq \#_i A$, which induces the equality.

%\hline
%(symmetrie fall:)\\
Assume that $\#_{A_{i+1}} B - \#_{A_{i+1}}\{\lambda_1\} < \#_{A_{i+1}} A$. Since $|A| = |B|$ this means right of $A_{i+1}$ there is positioned at least one more item $B_{i+1} \in B$. By our assumption we have $\#_{B_{i+1}} A - \#_{B_i} A \geq 2$. By equality (\ref{align:xPositionB}) it follows that between $B_i$ and $B_{i+1}$ there are positioned at least two items $c', c' \in c$ and at least one item $a' \in a$ and $b' \in b$, where $c'$ is positioned left of $c''$. We will now see how these items have to be arranged:
%Since $\#_{A_{i}} B = \#_{A_{i+1}} B$, equation (\ref{align:xPositionA}) ensues that between $A_i$ and $A_{i+1}$ there is no other item positioned.
%Equation (\ref{align:xPositionA}) and (\ref{align:xPositionB}) demand
%\[\#_{B_i} b \overset{(\ref{align:xPositionB})}{=} \#_{B_i} a \overset{(\ref{align:xPositionB})}{\geq} \#_{B_i} A = \#_{A_i} A = \#_{A_i} B -1 = \#_{A_{i+1}} B -1 \overset{(\ref{align:xPositionA})}{=}\#_{A_{i+1}} a \overset{(\ref{align:xPositionA})}{=}\#_{A_{i+1}} b.\]
%Therefore the items $a_i',a_{i+1}', b_i'$ and $b_{i+1}'$ have to be positioned right of $A_{i+1}$. 
%As a result we have 
%\[\#_{b_i'} c \overset{(\ref{align:xPositionb})}{=} \#_{b_i'} A \geq \#_{B_i} A +2  \overset{(\ref{align:xPositionB})}{=} \#_{B_i} c +2\]
%Hence $c_i'$ and $c_{i+1}'$ have to be placed left of $b_i'$. 
%Furthermore we have 
%\[\#_{a_i'} c \overset{(\ref{align:xPositiona})}{=} \#_{a_i'} B = \#_{A_i} B \overset{(\ref{align:xPositionA})}{=} \#_{A_i} c.\]
%This requires that $c_i'$ and $c_{i+1}'$ have to be placed left of $A_i$ or right of $a_{i+1}$. Since it holds that 
%\[\#_{c_{i+1}'} a = \#_{c_{i+1}'} b = \#_{B_i} b = \#_{B_i} a ,\]
%$c_{i+1}$ can not be placed right of $a_{i+1}$ and therefore has to be positioned left of $A_i$.
%To this point we have deduced that the packing has to look as follows: From left to right we see on slot 3 the items $B_i, c_i', c_{i+1}', A_i, A_{i+1}, b_{i}', b_{i+1}'$ (ignoring the items in $\delta$). Similar as before we can argue that this is not feasible. We have the following probperties:
%\[\#_{B_i} c \overset{(\ref{align:xPositionB})}{\geq} \#_{B_i} b = \#_{A_i} b \overset{(\ref{align:xPositionA})}{=} \#_{A_i} c -1 \geq \#_{B_i} c +1\]
%where the not marked (in)equalities originate from the deduced form of the packing. Since $\#_{B_i} c < \#_{B_i} c +1$ it follows that $\#_{A_{i+1}} B - \#_{A_{i+1}}\{\lambda_1\} = \#_{A_{i+1}} A$ .
First we know that $a'$ has to be scheduled between $c'$ and $c''$, since
\[\#_{a'} c =_{(\ref{align:xPositiona})} \#_{a'} B =_S \#_{B_i} B +1 =_{(\ref{align:AB})} \#_{B_i} A +1 =_{(\ref{align:xPositionB})} \#_{B_i} c +1.\] 
Furthermore, we know that  $A_i$ and $A_{i+1}$ have to be scheduled between $c'$ and $c''$ as well, since
\[\#_{A_{i}} c =_{(\ref{align:xPositionA})} \#_{A_{i}} B =_S \#_{B_i} B +1 =_{(\ref{align:AB})} \#_{B_i} A +1 =_{(\ref{align:xPositionB})} \#_{B_i} c +1\] 
and
\[\#_{A_{i+1}} c =_{(\ref{align:xPositionA})} \#_{A_{i+1}} B =_S \#_{B_i} B +1 =_{(\ref{align:AB})} \#_{B_i} A +1 =_{(\ref{align:xPositionB})} \#_{B_i} c +1.\] 
As a consequence, we can deduce that there is a job $b' \in b$ which is scheduled between $c'$ and $c''$, since
\[\#_{c''} b =_{(\ref{align:xPositionc})} \#_{c''} a =_S \#_{c'} a +1 =_{(\ref{align:xPositionc})} \#_{c'} b +1\] 
We know that about this $b'$ that 
\[\#_{b'} A =_{(\ref{align:xPositionb})} \#_{b'} c =_S \#_{B_{i}} c +1 =_{(\ref{align:xPositionB})} \#_{B_{i}} A +1, \]
so $b'$ has to be scheduled between $A_i$ and $A_{i+1}$. To this point we have deduced that the jobs are scheduled in the following order: $B_i, c', A_i, b', A_{i+1}, c'', B_{i+1}$. However, this schedule is invalid, since 
\[\#_{A_{i}} b =_{(\ref{align:xPositionA})} \#_{A_{i}} B - \#_{A_{i}} \{\lambda_1\} =_S  \#_{A_{i+1}} B - \#_{A_{i+1}} \{\lambda_1\} =_{(\ref{align:xPositionA})} \#_{A_{i+1}} b =_S \#_{A_{i}} b +1.\]
As a consequence, we have $\#_{A_{i+1}} B - \#_{A_{i+1}}\{\lambda_1\} = \#_{A_{i+1}} A$.
\end{proof}

We now will conclude that the \textit{structure items} have to be arranged as in Figure \ref{fig:packingStructure}.

\begin{lma}
The structure items from the sets $A.B,a,b,c,\alpha,\beta,\delta$ and $\lambda$ have to be placed as the items in Figure \ref{fig:packingStructure}.
\end{lma}
\begin{proof}

A simple conclusion is, that the first item on slot 1 is the item $\lambda_1$ and items out of $A$ and $B$ are placed alternating. Now it follows directly from the equations (\ref{align:xPositionA}), (\ref{align:xPositionB}), (\ref{align:xPositiona}), (\ref{align:xPositionb}) and (\ref{equ:relationAB}), that the items in the sets $A$, $B$, $\alpha$, $\beta$, $a$ and $b$ can only be placed as shown in Figure \ref{fig:packingStructure}. ($A$ and $B$ are placed alternating. It follows that between two $A$ there alwas have to be exactly one $a$ and one $\alpha$ and between two $B$ there have to be always one $b$ and one $\beta$. If an item out of $b$ is placed $\# A = \beta$, the the order is $B,\beta,b,B,\beta ...$. ) the placement of the items in $A$, $B$, $\alpha$, $\beta$, $a$ and $b$ leafs no other chose to place the items in $c$ and $\delta$ as displayed. The items in $\gamma$ have to be positioned in the gaps between $a$ and $B$. We can w.l.o.g assume that they follow directly after an item out of $a$. If not the only possibility is that an \textit{partition item} is positioned between the item in $A$ and the item in $\gamma$. We can swap these two items, without generating an overlapping.


\end{proof}
